Efficient Out-of-Distribution Detection of Melanoma with Wavelet-based Normalizing Flows

Melanoma is a serious form of skin cancer with high mortality rate at later stages. Fortunately, when detected early, the prognosis of melanoma is promising and malignant melanoma incidence rates are relatively low. As a result, datasets are heavily imbalanced which complicates training current state-of-the-art supervised classification AI models. We propose to use generative models to learn the benign data distribution and detect Out-of-Distribution (OOD) malignant images through density estimation. Normalizing Flows (NFs) are ideal candidates for OOD detection due to their ability to compute exact likelihoods. Nevertheless, their inductive biases towards apparent graphical features rather than semantic context hamper accurate OOD detection. In this work, we aim at using these biases with domain-level knowledge of melanoma, to improve likelihood-based OOD detection of malignant images. Our encouraging results demonstrate potential for OOD detection of melanoma using NFs. We achieve a 9% increase in Area Under Curve of the Receiver Operating Characteristics by using wavelet-based NFs. This model requires significantly less parameters for inference making it more applicable on edge devices. The proposed methodology can aid medical experts with diagnosis of skin-cancer patients and continuously increase survival rates. Furthermore, this research paves the way for other areas in oncology with similar data imbalance issues.

==> app/isic.tex <==
\section{Example images of the ISIC dataset}\label{app:isic}
We present a few benign and malignant Melanoma images from the ISIC dataset in Figure~\ref{fig:isic}.
\begin{figure}
\centering
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{figs/benign_images.png}
  \caption{Benign}
  \label{fig:sub1}
\end{subfigure}%
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{figs/malignant_images.png}
  \caption{Malignant}
  \label{fig:sub2}
\end{subfigure}
\caption{Example Melanoma images of the ISIC dataset}
\label{fig:isic}
\end{figure}

==> app/masking.tex <==
\section{Masking strategies}\label{app:masking}
Several methods can be used in the coupling layers to split the latent representations. By default, GLOW uses affine coupling. However, this can be replaced with any other masking strategy. We have experimented with checkerboard, cycle, horizontal and radial masking in the coupling steps of Wavelet Flow. For OOD detection, we have not witnessed any gain in ROC performance. Nevertheless, for completeness, we depict the different masking strategies in Figure~\ref{fig:masking}.

\begin{figure}
\centering
\includegraphics[width=0.7\linewidth]{figs/masking-strats.png}
\captionof{figure}{Various masking strategies are depicted. The masks are changed after each coupling flow step. The white area indicates the input of the $s,t$-network, which predicts parameters for the masked area in black. Grey areas are disregarded in the coupling process.}
\label{fig:masking}
\end{figure}

==> app/ood_wavelet.tex <==
\section{Out-of-distribution detection with the wavelet coefficient magnitudes}\label{app:wcodd}
Here, we consider the mean of the absolute wavelet coefficients at each decomposition scale. This, to investigate if an alternative such as using a generative model is needed. It is observed that the benign and malignant images are distinguishable per decomposition scale. However, the two likelihood densities are almost completely indistinguishable when averaged over all relevant decomposition scales.
\begin{figure}
\centering
\includegraphics[width=\linewidth]{figs/no-dl.png}
\captionof{figure}{The mean of the absolute wavelet coefficients per decomposition scale.}
\label{fig:nodl}
\end{figure}
\begin{figure}
\centering
\hspace{2em}\includegraphics[width=0.9\linewidth]{figs/no-dl-avg2.png}
\captionof{figure}{The mean of the absolute wavelet coefficients averaged over the decomposition scales.}
\label{fig:nodl2}
\end{figure}

==> app/training.tex <==
\section{Architectural and training details}\label{app:trainingdetails}
Four our experiments, we make use of the GLOW~\cite{kingma2018glow} and Wavelet Flow~\cite{yu2020wavelet} architecture. We use Glow in the multi-scale architecture (see Section 3.6 of Dinh~\textit{et al.}~\cite{dinh2016density}). Here, $K$ steps of the flow are preceded by a squeeze layer and split after the flow steps. One part of the split latent variable will continue to be subject to the flow steps while the other remains unchanged. This will be performed $L$ times. When $L$ is equal to one, no squeezing or splitting occurs. The $s$ and $t$ parameters in the coupling flow are obtained through a three-layer convolution neural network (CNN), with hidden dimensions of 256. We have not used a particular conditioning network for Wavelet Flow. The $s,t$-network is directly conditioned on the low-frequency images concatenated with the latent representations.

We make use of data augmentation such as random rotation, scaling, translation and shear. See Table~\ref{tab:aug} for details. All experiments have been performed with 128x128 pixel images and with a learning rate of $1e^{-4}$. After each epoch, the average likelihood of the complete training set is calculated and used for early stopping. If this number did not decrease after 10 epochs, training was stopped.

\begin{table}
\centering
\begin{tabular}{lcc} 
\toprule
\textbf{Random augmentation}  & Min & Max \\
\hline
Rotation & -180 & 180 \\
Translation & -0.1 & 0.1 \\
Scaling & 0.9 & 1.1 \\
Shear (x and y) & -10 & 10 \\
\bottomrule
\end{tabular}
\caption{Data augmentation settings}\label{tab:aug}
\end{table}


